From Fluent Text to Ontology-Compatible Definitions: A Quality-Control Agentic Workflow

Biomedical ontologies are structured knowledge systems that must evolve continuously to represent newly emerging knowledge, but their manual maintenance remains time-consuming and laborintensive. Textual definitions are especially costly because they must be readable to humans and compatible with controlled entities, relations, and logical constraints. Large language models (LLMs) offer a promising way to assist ontology engineering tasks, including definition generation. However, textual plausibility does not guarantee knowledge-system compatibility. A generated definition may be fluent and close to a reference definition, yet still fail to ground its implied entities or violate ontology-level constraints. Directly inserting such definitions into ontology libraries may therefore introduce entity-level hallucinations and logical inconsistencies. To address this problem, we propose two structured-knowledge incompatibility metrics, Entity Error Rate (EER) and Logical Inconsistency Rate (LIR), to quantify entity grounding and logical consistency for LLM-generated ontology definitions. We further develop an agentic quality-control (QC) workflow that treats definition generation as an iterative process rather than a direct decoding step: it generates definitions, extracts axioms, checks entity existence and logical consistency, and uses the resulting diagnostics to drive repair loops. Comprehensive experiments on Disease Ontology, Uberon Ontology, and Uberon-ConstraintStress demonstrate that EER and LIR complement conventional reference-based metrics by evaluating whether generated content can be grounded and checked inside the target ontology. The workflow effectively decreases EER while maintaining strong conventional text-generation performance. LIR further exposes sparse ontology-level logical failures that are invisible to text similarity metrics, although their repair remains limited.

==> chap00_abstract.tex <==
\begin{abstract}
    Biomedical ontologies are structured knowledge systems that must evolve
    continuously to represent newly emerging knowledge, but their manual
    maintenance remains time-consuming and labor-intensive.  Textual
    definitions are especially costly because they must be readable to humans
    and compatible with controlled entities, relations, and logical
    constraints.  Large language models (LLMs) offer a promising way to assist
    ontology engineering tasks, including definition generation.  However,
    textual plausibility does not guarantee knowledge-system compatibility.  A
    generated definition may be fluent and close to a reference definition, yet
    still fail to ground its implied entities or violate ontology-level
    constraints.  Directly inserting such definitions into ontology libraries
    may therefore introduce entity-level hallucinations and logical
    inconsistencies.
    To address this problem, we propose two structured-knowledge incompatibility
    metrics, Entity Error Rate (EER) and Logical Inconsistency Rate (LIR), to
    quantify entity grounding and logical consistency for LLM-generated
    ontology definitions.  We further develop an agentic quality-control (QC)
    workflow that treats definition generation as an iterative process rather
    than a direct decoding step: it generates definitions, extracts axioms,
    checks entity existence and logical consistency, and uses the resulting
    diagnostics to drive repair loops.  Comprehensive experiments on Disease
    Ontology, Uberon Ontology, and Uberon-Constraint-Stress demonstrate that
    EER and LIR complement conventional reference-based metrics by evaluating
    whether generated content can be grounded and checked inside the target
    ontology.  The workflow effectively decreases EER while maintaining strong
    conventional text-generation performance.  LIR further exposes sparse
    ontology-level logical failures that are invisible to text similarity
    metrics, although their repair remains limited.  The workflow source code
    and data are publicly available at:
    \url{
        ScrubbedForBlindReview
    }.
\end{abstract}


==> tables/text_generation_scores.tex <==
\begin{table*}[t]
    \centering
    \scriptsize
    \caption{Conventional text-generation scores for the same model-loop
    settings shown in \Cref{fig:result:eer}.  EER is shown in
    \Cref{fig:result:eer}, and LIR is reported separately in
    \Cref{tab:result:lir}.}
    \label{tab:result:main}
    \setlength{\tabcolsep}{3pt}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{lllccccc}
        \toprule
        Test setting & Model & Loop setting & Token F1 & ROUGE-L & BLEU-2 & BERT-F1 & Cosine \\
        \midrule
        DO 2024 & Qwen2.5-14B & Base, no loop & 0.283 & 0.222 & 0.107 & 0.608 & 0.664 \\
        DO 2024 & Qwen2.5-14B & Base, existence loop & \textbf{0.293} & \textbf{0.236} & \textbf{0.118} & \textbf{0.619} & \textbf{0.676} \\
        DO 2024 & Qwen2.5-14B & LoRA, no loop & \textbf{0.588} & 0.579 & 0.380 & 0.731 & 0.766 \\
        DO 2024 & Qwen2.5-14B & LoRA, existence loop & 0.588 & \textbf{0.579} & \textbf{0.381} & \textbf{0.731} & \textbf{0.766} \\
        DO 2024 & Llama-3.1-8B & Base, no loop & 0.310 & 0.240 & 0.115 & 0.593 & 0.642 \\
        DO 2024 & Llama-3.1-8B & Base, existence loop & \textbf{0.320} & \textbf{0.244} & \textbf{0.123} & \textbf{0.608} & \textbf{0.656} \\
        DO 2024 & Llama-3.1-8B & LoRA, no loop & 0.580 & 0.562 & \textbf{0.372} & 0.725 & 0.764 \\
        DO 2024 & Llama-3.1-8B & LoRA, existence loop & \textbf{0.580} & \textbf{0.562} & 0.372 & \textbf{0.725} & \textbf{0.764} \\
        \midrule
        DO 2025 & Qwen2.5-14B & Base, no loop & 0.327 & 0.253 & 0.143 & 0.636 & \textbf{0.688} \\
        DO 2025 & Qwen2.5-14B & Base, existence loop & \textbf{0.331} & \textbf{0.260} & \textbf{0.148} & \textbf{0.636} & 0.687 \\
        DO 2025 & Qwen2.5-14B & LoRA, no loop & 0.606 & 0.602 & 0.399 & 0.739 & 0.771 \\
        DO 2025 & Qwen2.5-14B & LoRA, existence loop & \textbf{0.606} & \textbf{0.602} & \textbf{0.399} & \textbf{0.739} & \textbf{0.771} \\
        DO 2025 & Llama-3.1-8B & Base, no loop & 0.345 & 0.257 & 0.139 & 0.611 & 0.658 \\
        DO 2025 & Llama-3.1-8B & Base, existence loop & \textbf{0.348} & \textbf{0.260} & \textbf{0.144} & \textbf{0.615} & \textbf{0.659} \\
        DO 2025 & Llama-3.1-8B & LoRA, no loop & 0.608 & 0.605 & 0.396 & 0.727 & 0.759 \\
        DO 2025 & Llama-3.1-8B & LoRA, existence loop & \textbf{0.608} & \textbf{0.605} & \textbf{0.396} & \textbf{0.727} & \textbf{0.759} \\
        \midrule
        Uberon 2024 & Qwen2.5-14B & Base, no loop & \textbf{0.428} & \textbf{0.353} & \textbf{0.203} & 0.663 & 0.717 \\
        Uberon 2024 & Qwen2.5-14B & Base, existence loop & 0.425 & 0.351 & 0.200 & \textbf{0.664} & \textbf{0.717} \\
        Uberon 2024 & Qwen2.5-14B & LoRA, no loop & 0.428 & 0.374 & 0.228 & \textbf{0.699} & \textbf{0.742} \\
        Uberon 2024 & Qwen2.5-14B & LoRA, existence loop & \textbf{0.431} & \textbf{0.378} & \textbf{0.230} & 0.699 & 0.742 \\
        Uberon 2024 & Llama-3.1-8B & Base, no loop & 0.409 & \textbf{0.332} & 0.175 & 0.649 & \textbf{0.698} \\
        Uberon 2024 & Llama-3.1-8B & Base, existence loop & \textbf{0.409} & 0.331 & \textbf{0.176} & \textbf{0.650} & 0.698 \\
        Uberon 2024 & Llama-3.1-8B & LoRA, no loop & 0.478 & 0.421 & 0.249 & 0.695 & 0.735 \\
        Uberon 2024 & Llama-3.1-8B & LoRA, existence loop & \textbf{0.484} & \textbf{0.424} & \textbf{0.257} & \textbf{0.701} & \textbf{0.743} \\
        \midrule
        Uberon 2025 & Qwen2.5-14B & Base, no loop & \textbf{0.408} & \textbf{0.346} & \textbf{0.190} & \textbf{0.659} & \textbf{0.702} \\
        Uberon 2025 & Qwen2.5-14B & Base, existence loop & 0.401 & 0.335 & 0.178 & 0.645 & 0.685 \\
        Uberon 2025 & Qwen2.5-14B & LoRA, no loop & 0.420 & 0.366 & 0.201 & \textbf{0.670} & \textbf{0.703} \\
        Uberon 2025 & Qwen2.5-14B & LoRA, existence loop & \textbf{0.421} & \textbf{0.367} & \textbf{0.202} & 0.670 & 0.703 \\
        Uberon 2025 & Llama-3.1-8B & Base, no loop & 0.393 & 0.319 & 0.173 & 0.653 & 0.691 \\
        Uberon 2025 & Llama-3.1-8B & Base, existence loop & \textbf{0.404} & \textbf{0.322} & \textbf{0.178} & \textbf{0.654} & \textbf{0.693} \\
        Uberon 2025 & Llama-3.1-8B & LoRA, no loop & \textbf{0.436} & 0.344 & 0.192 & \textbf{0.678} & \textbf{0.712} \\
        Uberon 2025 & Llama-3.1-8B & LoRA, existence loop & 0.435 & \textbf{0.346} & \textbf{0.195} & 0.675 & 0.709 \\
        \midrule
        Uberon-Constraint-Stress & Qwen2.5-14B & Base, no loop & 0.307 & 0.246 & 0.115 & \textbf{0.602} & \textbf{0.644} \\
        Uberon-Constraint-Stress & Qwen2.5-14B & Base, existence loop & \textbf{0.307} & \textbf{0.247} & \textbf{0.116} & 0.602 & 0.644 \\
        Uberon-Constraint-Stress & Qwen2.5-14B & LoRA, no loop & \textbf{0.416} & \textbf{0.379} & \textbf{0.242} & \textbf{0.674} & \textbf{0.712} \\
        Uberon-Constraint-Stress & Qwen2.5-14B & LoRA, existence loop & 0.410 & 0.373 & 0.237 & 0.669 & 0.707 \\
        Uberon-Constraint-Stress & Llama-3.1-8B & Base, no loop & \textbf{0.320} & \textbf{0.257} & \textbf{0.117} & 0.603 & 0.644 \\
        Uberon-Constraint-Stress & Llama-3.1-8B & Base, existence loop & 0.319 & 0.255 & 0.116 & \textbf{0.603} & \textbf{0.644} \\
        Uberon-Constraint-Stress & Llama-3.1-8B & LoRA, no loop & \textbf{0.409} & \textbf{0.368} & \textbf{0.226} & \textbf{0.664} & \textbf{0.702} \\
        Uberon-Constraint-Stress & Llama-3.1-8B & LoRA, existence loop & 0.404 & 0.363 & 0.220 & 0.657 & 0.695 \\
        \bottomrule
    \end{tabular}}
\end{table*}


==> tables/text_generation_scores_all_loop.tex <==
\begin{table*}[t]
    \centering
    \scriptsize
    \caption{Conventional text-generation scores comparing direct generation
    with the full QC workflow.  Each pair compares no-loop generation with
    the corresponding all-loop setting; bold marks the higher score within
    each pair, with ties assigned to the all-loop setting.}
    \label{tab:app:all_loop_text}
    \setlength{\tabcolsep}{3pt}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{lllccccc}
        \toprule
        Test setting & Model & Loop setting & Token F1 & ROUGE-L & BLEU-2 & BERT-F1 & Cosine \\
        \midrule
        DO 2024 & Qwen2.5-14B & Base, no loop & 0.283 & 0.222 & 0.107 & 0.608 & 0.664 \\
        DO 2024 & Qwen2.5-14B & Base, all loops & \textbf{0.293} & \textbf{0.236} & \textbf{0.118} & \textbf{0.619} & \textbf{0.676} \\
        DO 2024 & Qwen2.5-14B & LoRA, no loop & \textbf{0.588} & 0.579 & 0.380 & 0.731 & 0.766 \\
        DO 2024 & Qwen2.5-14B & LoRA, all loops & 0.588 & \textbf{0.579} & \textbf{0.381} & \textbf{0.731} & \textbf{0.766} \\
        DO 2024 & Llama-3.1-8B & Base, no loop & 0.310 & 0.240 & 0.115 & 0.593 & 0.642 \\
        DO 2024 & Llama-3.1-8B & Base, all loops & \textbf{0.320} & \textbf{0.244} & \textbf{0.123} & \textbf{0.608} & \textbf{0.656} \\
        DO 2024 & Llama-3.1-8B & LoRA, no loop & 0.580 & 0.562 & \textbf{0.372} & 0.725 & 0.764 \\
        DO 2024 & Llama-3.1-8B & LoRA, all loops & \textbf{0.580} & \textbf{0.562} & 0.372 & \textbf{0.725} & \textbf{0.764} \\
        \midrule
        DO 2025 & Qwen2.5-14B & Base, no loop & 0.327 & 0.253 & 0.143 & 0.636 & \textbf{0.688} \\
        DO 2025 & Qwen2.5-14B & Base, all loops & \textbf{0.331} & \textbf{0.260} & \textbf{0.148} & \textbf{0.636} & 0.687 \\
        DO 2025 & Qwen2.5-14B & LoRA, no loop & 0.606 & 0.602 & 0.399 & 0.739 & 0.771 \\
        DO 2025 & Qwen2.5-14B & LoRA, all loops & \textbf{0.606} & \textbf{0.602} & \textbf{0.399} & \textbf{0.739} & \textbf{0.771} \\
        DO 2025 & Llama-3.1-8B & Base, no loop & 0.345 & 0.257 & 0.139 & 0.611 & 0.658 \\
        DO 2025 & Llama-3.1-8B & Base, all loops & \textbf{0.348} & \textbf{0.260} & \textbf{0.144} & \textbf{0.615} & \textbf{0.659} \\
        DO 2025 & Llama-3.1-8B & LoRA, no loop & 0.608 & 0.605 & 0.396 & 0.727 & 0.759 \\
        DO 2025 & Llama-3.1-8B & LoRA, all loops & \textbf{0.608} & \textbf{0.605} & \textbf{0.396} & \textbf{0.727} & \textbf{0.759} \\
        \midrule
        Uberon 2024 & Qwen2.5-14B & Base, no loop & \textbf{0.428} & \textbf{0.353} & \textbf{0.203} & 0.663 & 0.717 \\
        Uberon 2024 & Qwen2.5-14B & Base, all loops & 0.425 & 0.351 & 0.200 & \textbf{0.664} & \textbf{0.717} \\
        Uberon 2024 & Qwen2.5-14B & LoRA, no loop & 0.428 & 0.374 & 0.228 & \textbf{0.699} & \textbf{0.742} \\
        Uberon 2024 & Qwen2.5-14B & LoRA, all loops & \textbf{0.431} & \textbf{0.378} & \textbf{0.230} & 0.699 & 0.742 \\
        Uberon 2024 & Llama-3.1-8B & Base, no loop & 0.409 & \textbf{0.332} & 0.175 & 0.649 & \textbf{0.698} \\
        Uberon 2024 & Llama-3.1-8B & Base, all loops & \textbf{0.409} & 0.331 & \textbf{0.176} & \textbf{0.650} & 0.698 \\
        Uberon 2024 & Llama-3.1-8B & LoRA, no loop & 0.478 & 0.421 & 0.249 & 0.695 & 0.735 \\
        Uberon 2024 & Llama-3.1-8B & LoRA, all loops & \textbf{0.484} & \textbf{0.424} & \textbf{0.257} & \textbf{0.701} & \textbf{0.743} \\
        \midrule
        Uberon 2025 & Qwen2.5-14B & Base, no loop & \textbf{0.408} & \textbf{0.346} & \textbf{0.190} & \textbf{0.659} & \textbf{0.702} \\
        Uberon 2025 & Qwen2.5-14B & Base, all loops & 0.401 & 0.335 & 0.178 & 0.645 & 0.685 \\
        Uberon 2025 & Qwen2.5-14B & LoRA, no loop & 0.420 & 0.366 & 0.201 & \textbf{0.670} & \textbf{0.703} \\
        Uberon 2025 & Qwen2.5-14B & LoRA, all loops & \textbf{0.421} & \textbf{0.367} & \textbf{0.202} & 0.670 & 0.703 \\
        Uberon 2025 & Llama-3.1-8B & Base, no loop & 0.393 & 0.319 & 0.173 & 0.653 & 0.691 \\
        Uberon 2025 & Llama-3.1-8B & Base, all loops & \textbf{0.404} & \textbf{0.322} & \textbf{0.178} & \textbf{0.654} & \textbf{0.693} \\
        Uberon 2025 & Llama-3.1-8B & LoRA, no loop & \textbf{0.436} & 0.344 & 0.192 & \textbf{0.678} & \textbf{0.712} \\
        Uberon 2025 & Llama-3.1-8B & LoRA, all loops & 0.435 & \textbf{0.346} & \textbf{0.195} & 0.675 & 0.709 \\
        \midrule
        Uberon-Constraint-Stress & Qwen2.5-14B & Base, no loop & 0.307 & 0.246 & 0.115 & \textbf{0.602} & \textbf{0.644} \\
        Uberon-Constraint-Stress & Qwen2.5-14B & Base, all loops & \textbf{0.307} & \textbf{0.247} & \textbf{0.116} & 0.602 & 0.644 \\
        Uberon-Constraint-Stress & Qwen2.5-14B & LoRA, no loop & \textbf{0.416} & \textbf{0.379} & \textbf{0.242} & \textbf{0.674} & \textbf{0.712} \\
        Uberon-Constraint-Stress & Qwen2.5-14B & LoRA, all loops & 0.410 & 0.373 & 0.237 & 0.669 & 0.707 \\
        Uberon-Constraint-Stress & Llama-3.1-8B & Base, no loop & \textbf{0.320} & \textbf{0.257} & \textbf{0.117} & 0.603 & 0.644 \\
        Uberon-Constraint-Stress & Llama-3.1-8B & Base, all loops & 0.319 & 0.255 & 0.116 & \textbf{0.603} & \textbf{0.644} \\
        Uberon-Constraint-Stress & Llama-3.1-8B & LoRA, no loop & \textbf{0.409} & \textbf{0.368} & \textbf{0.226} & \textbf{0.664} & \textbf{0.702} \\
        Uberon-Constraint-Stress & Llama-3.1-8B & LoRA, all loops & 0.404 & 0.363 & 0.220 & 0.657 & 0.695 \\
        \bottomrule
    \end{tabular}}
\end{table*}

